Understanding the Role of Textual Prompts in LLM for Time Series Forecasting: an Adapter View

In the burgeoning domain of Large Language Models (LLMs), there is a growing interest in applying LLM to time series forecasting, with multiple studies focused on leveraging textual prompts to further enhance the predictive prowess. This study aims to understand how and why the integration of textual prompts into LLM can effectively improve the prediction accuracy of time series, which is not obvious at the glance, given the significant domain gap between texts and time series. Our extensive examination leads us to believe that (a) adding text prompts is roughly equivalent to introducing additional adapters, and (b) It is the introduction of learnable parameters rather than textual information that aligns the LLM with the time series forecasting task, ultimately enhancing prediction accuracy. Inspired by this discovery, we developed four adapters that explicitly address the gap between LLM and time series, and further improve the prediction accuracy. Overall,our work highlights how textual prompts enhance LLM accuracy in time series forecasting and suggests new avenues for continually improving LLM-based time series analysis.

==> sections/1_introduction.tex <==
\section{Introduction}\label{sec:introduction}

Time series analysis is a fundamental problem that has played an important role in many real-world applications \cite{wen2022robust}, ranging from energy, weather, traffic to economics.
In the past few years, following the significant success in NLP \cite{vaswani2017attention} and CV \cite{bao2022beit}, transformer-based models have become widely prevalent in time-series tasks, demonstrating promising results \cite{zhou2022fedformer, wu2021autoformer, Patchformer, zhou2021informer, dcdetector, wen2022transformers}.

In the last couple of years, we have witnessed the rapid development of foundation models in NLP~\cite{OpenAI2023GPT4TR, Touvron2023LLaMAOA} and CV~\cite{kirillov2023segany}. Recently, researchers have explored constructing foundational models for time series tasks~\cite{garza2023timegpt1, rasul2024lagllama}. However, time series often face challenges such as insufficient data volume and significant disparities across different domains.
An effective solution is to transfer pre-trained language or vision models to time series data and \cite{zhou2023onefitsall} has demonstrated that pre-trained transformers can provide a universal representation with transferable capabilities.

Another, even more impressive method is to directly use linguistic guidance for a large language models (LLM) to yield precise results for time series tasks.
Most of the research in this field focuses on designing an effective prompts and aligning the word embeddings of LLM with time series embeddings \cite{jin2024timellm, xue2023promptcast, Jia2024GPT4MTSPL}.
However, there is currently limited in-depth analysis of \textbf{how linguistic information affects time series forecasting}, and whether performance improvements are predominantly influenced by the introduction of more parameters.

In order to conduct an initial exploration of this issue, we present a formal critique of the advantages of utilizing linguistic information and design various scenarios and empirical verifications to evaluate the improvements brought about by existing methods.
And we have discovered that \textbf{incorporating linguistic information does not yield significant practical benefits}. Instead, \textbf{the observed improvements can be primarily attributed to the introduction of more learnable parameters, which can be viewed as implicit adapters}.
To further validate this conclusion, we propose four explicit adapters to incorporate time specific information, which also has the potential to significantly enhance performance.
Based on our analyses and conclusions, we also encourage the community to delve deeper into investigating the impact of linguistic information in large language models on time series analysis.

Here we summarize our key contributions as follows:
\begin{enumerate}
    \item Our analysis and empirical evidence have shown that current methods of integrating linguistic information into large language models (LLMs) fail to offer tangible benefits. Instead, they inadvertently insert implicit adapters, driving any observed improvements.
    \item To further validate the conclusion regarding implicit adapters, we propose the introduction of explicit adapters into OFA \cite{zhou2023onefitsall}, including temporal, channel, frequency and anomaly adapters, specifically designed for time series. The results substantiate that explicit adapters, rather than linguistic information, can also yield performance improvements across various time series tasks.
\end{enumerate}

The remainder of this paper is structured as follows. Section 2 briefly summarizes the related work of LLM applications for time series. Section 3 gives the analysis from information theory and empirical study to validate the argument that the performance improvement is not primarily attributed to linguistic information. Section 4 presents the proposed explicit adapters for time series. In Section 5, we conduct a thorough and extensive evaluation of the performance of time series analysis using our proposed method. Finally, in Section 6, we discuss our results and future directions.

==> tables/ablation_gate.tex <==
\begin{table}
\caption{Ablation on select gate. The list displays the learned coefficients, which represent the gate coefficient for each layer.}
\label{tab:ablation_gate}
\begin{center}
\begin{tabular}{c|ccc|c}
\hline

\multirow{2}{*}{Datasets}
& \multicolumn{3}{c|}{Learned Coefficients} & \multirow{2}{*}{MSE} \\
& Temporal & Channel & Frequency \\

\toprule

ETTh1 720 & [1,0,0,1,0,0] & [1,1,1,0,1,1] & [1,1,1,1,1,1] & 0.432 \\
ETTh2 96  & [1,0,1,1,0,0] & [1,1,0,0,1,1] & [1,1,1,1,0,1] & 0.269 \\
ETTh2 720 & [1,0,1,1,1,1] & [1,1,1,1,1,1] & [1,1,1,1,1,1] & 0.392 \\


\bottomrule

\end{tabular}
\end{center}
\end{table}

==> tables/anomaly.tex <==
\begin{table*}[h]
\caption{Anomaly detection task. We calculate the F1-score, Precision and Recall (as \%) for each dataset. A higher F1 indicates better performance. \textbf{Black}: best, \underline{Underline}: second best.}
\label{tab:anomaly}
\begin{center}
\begin{threeparttable}[b]
\begin{tabular}{cc|ccccccccc}
\toprule

% Methods &
% \multicolumn{3}{c|}{SMD} & \multicolumn{3}{c|}{MSL} & \multicolumn{3}{c|}{SMAP}& \multicolumn{3}{c|}{SWaT} &\multicolumn{3}{c|}{PSM} & Avg F1 \\
% Metrics&P&R&F1&P&R&F1&P&R&F1&P&R&F1&P&R&F1&\%  \\

\multicolumn{2}{c|}{{Methods}}&GPT2(6)-adapter&GPT2(6)-frozen&Anomaly\tnote{*}&TimeNet\tnote{**}&Anomaly(Rec)\tnote{***}&PatchTST&FEDformer&DLinear&Autoformer \\
\midrule
\multicolumn{2}{c|}{{Reconstruction}}&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark \\
\multicolumn{2}{c|}{{Discrepancy}}&\checkmark&-&\checkmark&-&-&-&-&-&- \\
\midrule

\multirow{3}{*}{\rotatebox{90}{$SMD$}}
&P&88.65&88.89&89.40&87.91&88.91&87.26&87.95&83.62&88.06 \\
&R&91.37&84.98&95.45&82.54&82.23&82.14&82.39&71.52&82.35 \\
&F1&\underline{89.99}&86.89&\textbf{92.33}&84.61&85.49&84.62&85.08&77.10&85.11 \\
\midrule

\multirow{3}{*}{\rotatebox{90}{$MSL$}}
&P&93.26&82.00&92.09&89.54&79.61&88.34&77.14&84.34&77.27 \\
&R&93.90&82.91&95.15&75.36&87.37&70.96&80.07&85.42&80.92 \\
&F1&\underline{93.58}&82.45&\textbf{93.59}&81.84&83.31&78.70&78.57&84.88&79.05 \\
\midrule

\multirow{3}{*}{\rotatebox{90}{$SMAP$}}
&P&95.43&90.60&94.13&90.14&91.85&90.64&90.47&92.32&90.40 \\
&R&98.38&60.95&99.40&56.40&58.11&55.46&58.10&55.41&58.62 \\
&F1&\textbf{96.88}&72.88&\underline{96.69}&69.39&71.18&68.82&70.76&69.26&71.12 \\
\midrule

\multirow{3}{*}{\rotatebox{90}{$SWaT$}}
&P&96.44&92.20&91.55&90.75&72.51&91.10&90.17&80.91&89.85 \\
&R&99.78&96.34&96.73&95.40&97.32&80.94&96.42&95.30&95.81 \\
&F1&\textbf{98.08}&\underline{94.23}&94.07&93.02&83.10&85.72&93.19&87.52&92.74 \\
\midrule

\multirow{3}{*}{\rotatebox{90}{$PSM$}}
&P&99.06&98.62&96.91&98.51&68.35&98.84&97.31&98.28&99.08 \\
&R&97.39&95.68&98.90&96.20&94.72&93.47&97.16&89.26&88.15 \\
&F1&\textbf{98.22}&97.13&\underline{97.89}&97.34&79.40&96.08&97.23&93.55&93.29 \\
\midrule

\multicolumn{2}{c|}{$Avg.\ F1$}&\textbf{95.35}&86.72&\underline{94.91}&85.24&80.50&82.79&84.97&82.46&84.26 \\
\midrule

% \multirow{2}{*}{\rotatebox{90}{Datasets}}

% \midrule
% GPT(6)&{\bf88.89}&{\bf84.98}&{\bf86.89}&82.00&{\bf82.91}&{\bf82.45}&{\bf90.60}&{\bf60.95}&{\bf72.88}&{\bf92.20}&{\bf96.34}&{\bf94.23}&{\bf98.62}&95.68&97.13&{\bf86.72}\\
% TimesNet &87.91&81.54&84.61&{\bf89.54}&75.36&81.84&90.14&56.40&69.39&90.75&95.40&93.02&98.51&{\bf96.20}&{\bf97.34}&85.24\\
% PatchTST&87.26&82.14&84.62&88.34&70.96&78.70&90.64&55.46&68.82&91.10&80.94&85.72&98.84&93.47&96.08&82.79\\
% FEDformer&87.95&82.39&85.08&77.14&80.07&78.57&90.47&58.10&70.76&90.17&96.42&93.19&97.31&97.16&97.23&84.97\\
% DLinear&83.62&71.52&77.10&84.34&85.42&84.88&92.32&55.41&69.26&80.91&95.30&87.52&98.28&89.26&93.55&82.46 \\
% Autoformer&88.06&82.35&85.11&77.27&80.92&79.05&90.40&58.62&71.12&89.85&95.81&92.74&99.08&88.15&93.29&84.26 \\
% Anomaly Transformer&88.91&82.23&85.49&79.61&87.37&83.31&91.85&58.11&71.18&72.51&97.32&83.10&68.35&94.72&79.40&80.50 \\

% \bottomrule

\end{tabular}

\begin{tablenotes}
\item[*] Anomaly represents Anomaly Transformer.
\item[**] We reproduce the results of TimesNet by \href{https://github.com/thuml/Time-Series-Library}{https://github.com/thuml/Time-Series-Library}.
\item[***] The joint criterion in Anomaly Transformer is replaced with reconstruction error.
\end{tablenotes}
\end{threeparttable}

\end{center}
\end{table*}

==> tables/gate_methods.tex <==
\begin{table}[h]
\caption{Different adapters for different datasets.}
\label{tab:gate_methods}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{c|ccc|c}
\hline

\multirow{2}{*}{Datasets}
& \multicolumn{3}{c|}{Adapters} & \multirow{2}{*}{MSE} \\
& Temporal & Channel & Frequency \\

\toprule

\multirow{3}{*}{ETTh1 96}
& \checkmark & - & - & 0.375 \\
& - & \checkmark & - & 0.373 \\
& - & - & \checkmark & \textbf{0.369} \\

\midrule

\multirow{3}{*}{ETTh2 96}
& \checkmark & - & - & \textbf{0.280} \\
& - & \checkmark & - & 0.285 \\
& - & - & \checkmark & 0.282 \\

\bottomrule

\end{tabular}
}
\end{center}
\end{table}
